MAGMA: An Optimization Framework for Mapping Multiple DNNs on Multiple Accelerator Cores

As Deep Learning continues to drive a variety of applications in edge and cloud data centers, there is a growing trend towards building large accelerators with several sub-accelerator cores/chiplets. This work looks at the problem of supporting multi-tenancy on such accelerators. In particular, we focus on the problem of mapping jobs from several DNNs simultaneously on an accelerator. Given the extremely large search space, we formulate the search as an optimization problem and develop an optimization framework called M3E. In addition, we develop a specialized optimization algorithm called MAGMA with custom operators to enable structured sample-efficient exploration. We quantitatively compare MAGMA with several state-of-the-art methods, black-box optimization, and reinforcement learning methods across different accelerator settings (large/small accelerators) and different sub-accelerator configurations (homogeneous/heterogeneous), and observe MAGMA can consistently find better mappings.

==> figure/app_dim.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/app_dim.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The dominant layers of three applications and the dimension definitions of different layer types. \textit{CONV}: K/C: size of output/input channels, Y/X: height/width of activations, R/S: height/width of weight. \textit{FC}: O: Output nodes, I: Input nodes, \textit{FC-E}: E: Embedding sizes.}
\vspace{-0.1cm}
\label{fig:app_dim}
\end{figure}




==> figure/encoding.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/encoding.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The encoding scheme of \framework.
}
%\TK{This table is still not very clear to me. The avg row is avg across the models. what does the Avg column mean? Avg across both accelerators? I think the avg column can be removed - and table font size will go up. The graphs are showing the avg anyway.}\FK{Yes, the column is showing Avg across accelerators. Removed.}}

\label{fig:encoding}
\end{figure}




==> figure/gene.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/gene.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The design genetic encoding and its decoding procedure.}
\vspace{-0.2cm}
\label{fig:gene}
\end{figure}




==> figure/operator.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/operator.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The genetic operators.}
\vspace{-0.2cm}
\label{fig:operator}
\end{figure}




==> figure/programmable.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/programmable.pdf}
\end{center}
\vspace{-0.1cm}
\caption{A mapping example on PEs arrays with different flexibility.}
\vspace{-0.2cm}
\label{fig:programmable}
\end{figure}




==> figure/s2_bar.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/s2_bar.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The latency of different scheduling methods on (a) Language traffic and (b) Recommendation traffic (S2, BW=1).}
\vspace{-0.2cm}
\label{fig:s2_bar}
\end{figure}




==> figure/s6.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/s6.pdf}
\end{center}
\vspace{-0.2cm}
\caption{The experiment results on a scale-up platform in S6, BW=256.}
\vspace{-0.4cm}
\label{fig:s6}
\end{figure}




==> figure/sat.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=1\linewidth]{Figures/sat.pdf}
\end{center}
\vspace{-0.2cm}
\caption{(a) The SAT convergence trace (Mix, S3, BW=1). (b) The definition of SAT.}
\vspace{-0.2cm}
\label{fig:sat}
\end{figure}




==> sections/09-Note.tex <==

Taking cue from prior efforts on heterogeneous scheduling in datacenters, we will explore popular heuristics (first-come first-serve, shortest-job first, round robin~\cite{gpu_fcfs,leutenegger1990performance}, ...) and optimization methods~\cite{nevergad} (such as sampling searches~\cite{halton, hammersley}, particle swarm optimization~\cite{pso_paper}, genetic algorithms~\cite{ga}, and reinforcement learning~\cite{reinforce}) for the mapper.

\cite{scarl} 70 secs per epoch and 500 epochs Intel(R)
Core(TM) i7-8700 CPU v.s. us 20 secs for 100 epochs
They made the assumption that the job sequence are similar. (For most RL-based method to work)
Most of the works are in a sense of job (a task with runtime and resource reuqiremnet), we are explore DNN layers, wheere the mapping and PEs matters.

==> sections/Cut-for-hpca-rebuttal.tex <==
\input{figure/bw_aloc_result}
\textbf{Analysis of found solutions.}
\subsection{Latency-BW Characteristics of DNNs}

==> table/cloud_table.tex <==


\begin{table}[h]

\centering
\caption{The experiment results on cloud platform on Heteto (S4) and Hetero BigLittle (S5) setting. }

\includegraphics[width=1\linewidth]{Figures/cloud_graph.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:cloud_table}
\end{table}


==> table/edge_bw_effect.tex <==


\begin{table}[h]

\centering
\caption{The latency decrease with the increase of BW budget on (a) S1 and (b) S2.}

\includegraphics[width=1\linewidth]{Figures/edge_bw_effect.pdf}
\vspace{-0.2cm}
\label{table:edge_bw_effect}
\end{table}


==> table/edge_table.tex <==


\begin{table*}[h]

\centering
\caption{The experiment results on fog node with (a) S1 and (b) S2 setting, and on cloud node on (c) S4 and (d) S5 setting. }

\includegraphics[width=1\linewidth]{Figures/edge_graph.pdf}
% Figures/edge_table.pdf
\vspace{-0.2cm}
\label{table:edge_table}
\end{table*}


==> table/model_table.tex <==


\begin{table}[h]

\centering
\caption{Models of different applications included in the experiments. }

\includegraphics[width=1\linewidth]{Figures/model_table.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:model_table}
\end{table}


==> table/model_table_latex.tex <==

\begin{table}[]
\caption{\it Evaluated DNNs in different Tasks.}
\scriptsize
% \begin{tabular}{|
% >{\columncolor[HTML]{EFEFEF}}c |l|}
\begin{tabular}{|>{\columncolor[HTML]{C0C0C0}}p{2.0em}|p{31em}|}
\hline
Task Type & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}DNN Models}                                                                                                                                   \\ \hline
Vision   & \makecell[l]{AlexNet~\cite{Alexnet}, DenseNet~\cite{densenet}, GoogleNet~\cite{Googlenet}, MnasNet~\cite{mnasnet}, \\ MobileNet-V2~\cite{sandler2018mobilenetv2},  ResNet50~\cite{Resnet}, ResNext50~\cite{resnext},  ResNet18~\cite{Resnet},\\  WideResNet50~\cite{Resnet}, SuffleNet-V2~\cite{zhang2018shufflenet},  SqueezeNet~\cite{squeezenet}, VGG16~\cite{vgg}  }                                                 \\ \hline
Lang & \makecell[l]{ALBERT~\cite{albert}, Bart~\cite{bart}, BERT~\cite{bert}, CamemBERT~\cite{camembert}, CTRL~\cite{ctrl_lang},\\ DistilBERT~\cite{sanh2019distilbert}, ELECTRA~\cite{electra}, FlauBERT~\cite{flaubert}, GPT2~\cite{gpt2}, GPT~\cite{gpt},\\ LongFormer~\cite{longformer}, MarianNMT~\cite{mariannmt}, MobileBERT~\cite{sun2020mobilebert}, Reformer~\cite{reformer}, \\ RetriBERT~\cite{retribert}, RoBERTa~\cite{roberta}, T5~\cite{t5}, TransformerXL~\cite{transformerxl}, XLM~\cite{xlm}, \\ XLM-RoBERTa~\cite{xlmroberta}, XLNet~\cite{xlnet}} \\ \hline
Recom    & \makecell[l]{DIN~\cite{din}, DIEN~\cite{dien},  DLRM-MLPerf~\cite{mlperf}, DLRM-large~\cite{dlrm_intel}, \\DLRM-small~\cite{dlrm}, WideDeep~\cite{widedeep}, DLRM-RMC1~\cite{deeprecsys}, DLRM-RMC2~\cite{deeprecsys} }                                                                                                         \\ \hline
\end{tabular}
\label{table:model_table}
\end{table}

==> table/programmable_table.tex <==


\begin{table}[t]

\centering
\caption{The traffic analysis of different level of flexibility and their latency performance. }

\includegraphics[width=1\linewidth]{Figures/programmable_table_graph.pdf}
% Figures/programmable_table.pdf
\vspace{-0.2cm}
\label{table:programmable_table}
\end{table}


==> table/runtime.tex <==


\begin{table}[h]

\centering
\caption{\hl{The comparisons of search time and the makespan speedup over heuristic methods. The statistics values are averaged across different settings (S1-S6) of different job categories. G-SHARP-transfer represents G-SHARP with transferred knowledge.} }

\includegraphics[width=1\linewidth]{Figures/runtime_table.pdf}
% Figures/cloud_table.pdf
\vspace{-0.5cm}
\label{table:runtime}
\end{table}


==> table/s3_s4_s5.tex <==
\begin{table*}[h]

\centering
\caption{(a) The averaged non-stall latency and the required BW of S3 (BigHomo), S4 (BigHetero), and S5 (BigLittleHetero) in different traffics. (b) The latency performance for S3, S4, and S5 in different traffics and BW. }

\includegraphics[width=1\linewidth]{Figures/s3_s4_s5_graph.pdf}
% Figures/s3_s4_s5.pdf
\vspace{-1cm}
\label{table:s3_s4_s5}
\end{table*}


==> table/s6.tex <==


\begin{table*}[h]

\centering
\caption{The experiment results on cloud platform on Scale-up (S6), BW=1. }

\includegraphics[width=1\linewidth]{Figures/s6.pdf}
\vspace{-0.2cm}
\label{table:s6_table}
\end{table*}


==> table/traffic_analysis.tex <==


\begin{table*}[h]

\centering
\caption{Traffic analysis of different applications. }

\includegraphics[width=1\linewidth]{Figures/traffic_analysis.pdf}
\vspace{-0.2cm}
\label{table:traffic_analysis}
\end{table*}


==> table/trf_1.tex <==


\begin{table}[t]

\centering
\caption{The knowledge transferring on Vision, S4 setting. All the values are noramalized by the values of Trf-100-ep of each columns. Raw is the latency without learning or transferred. Trf-0-ep is a direct transfer without retraining. Trf-1-ep is a transfer with one epoch of re-training, and likewise for Trf-30-ep and Trf-100-ep.Since we run all the optimization for 100 epochs, Trf-100-ep is similar to training from scratch. }

\includegraphics[width=0.7\linewidth]{Figures/trf_1.pdf}

\label{table:trf_1}
\end{table}


==> table/trf_2.tex <==


\begin{table}[h]

\centering
\caption{The knowledge transferring on (left) different setting of Mix traffics and (right) different traffic types. All the values are noramalized by the values of Trf-100-ep of each columns.}

\includegraphics[width=1\linewidth]{Figures/trf_2.pdf}

\label{table:trf_2}
\end{table}

